Scalable MatMul-free Language Modeling

Large Language Models (LLMs) have fundamentally altered how we approach scaling in machine learning. However, these models pose substantial computational and memory challenges, primarily due to the reliance on matrix multiplication (MatMul) within their attention and feed-forward (FFN) layers. We demonstrate that MatMul operations can be eliminated from LLMs while maintaining strong performance, even at billion-parameter scales. Our MatMul-free models, tested on models up to 2.7B parameters, are comparable to state-of-the-art pre-trained Transformers, and the performance gap narrows as model size increases. Our approach yields significant memory savings: a GPU-efficient implementation reduces memory consumption by up to 61% during training and over 10x during inference. When adapted for a multi-chip neuromorphic system, the model leverages asynchronous processing to achieve 4x higher throughput with 10x less energy than edge GPUs.

==> changes.tex <==
~~~ means fixed

- reduce abstract length (258 words to 200 words?)
~~~~ - Fig. 1: search emails for pic of Hala Point
    done
- CONSIDER: Visual depiction of Loihi Results
- Table 3 and Appendix chip: multi-chip, single-chip?
~~~ - Fix some aesthetic issues (pg 11) 
    fixed now
~~~ - Page 17: Broken reference. "The partitioning of the MMF model into Loihi-compatible neurons is shown 
    done

- Appendix: perhaps include more context on the FPGA results?
- final proofread

- take out "currently working on XYZ" mentions?

- Make sure abstract claims match the results claims (61\% savings, 10x during inference, 3x higher throughput, 2x less energy than edge GPUs, 25x less energy than server-class GPUs)

- Make sure introduction claims match the results claims (4.1 W at far beyond human readable throughput)
%%%%
% single-chip: 59 mJ/tokens * 71 tokens/sec = 4.1W
% multichip: 405*41.5=16.8W
% TF Jetson: 15*720=10.8W
%%%%

Loihi shit:
~~~- check section 5~~~
    good, but presents single-chip results
~~~- check section 6.5~~~
    good to go
- appendix
- fix appendix loihi graph figure
    

- Submit

- arXiv submit
- profit


==> sn-article-old-l2.tex <==
\section*{Old results table in Section 5.3}

\textcolor{red}{New results include a 20\% decrease in throughput since that's what the multi-chip results have shown us. Refer to the Overleaf version on July 12 for the full old results.}

\begin{table*}[h]
\caption{Throughput and energy efficiency for various transformer-based language models running on the NVIDIA Jetson Orin Nano compared to our MatMul-free LM running on Intel's Loihi 2. Comparing language models with at most 500M parameters. Metrics for Loihi 2 are estimated based on single-chip measurements.}
\centering
\begin{tabular}{l|llll|llll}
\toprule
 & \multicolumn{4}{l}{Throughput (tokens/sec)} & \multicolumn{4}{l}{Efficiency (mJ/token)} \\
\midrule
Generate & 500 & 1000 & 2000 & 4000 & 500 & 1000 & 2000 & 4000 \\
\midrule
Alireo-400M & 14.3 & 14.9 & 15.0 & 14.7 & 723 & 719 & 751 & 853 \\
% Pythia-410M & 21.4 & 22.3 & 23.9 & 22.4 & 530.3 & 560.8 & 597.5 & 730.6 \\
Qwen2-500M & 13.4 & 14.0 & 14.1 & 14.1 & 791 & 785 & 816 & 912 \\
% \textbf{Ours (370M)} & \textbf{21.6} & \textbf{21.6} & \textbf{21.6} & \textbf{21.6} & \textbf{223} & \textbf{223} & \textbf{223} & \textbf{223} \\
\textbf{Ours (370M)} & \textbf{71.3} & \textbf{71.3} & \textbf{71.3} & \textbf{71.3} & \textbf{59} & \textbf{59} & \textbf{59} & \textbf{59} \\
% Alireo-400M & 14.3 & 14.9 & 15.0 & 14.7 & 723.4 & 718.7 & 750.7 & 852.8 \\
% % Pythia-410M & 21.4 & 22.3 & 23.9 & 22.4 & 530.3 & 560.8 & 597.5 & 730.6 \\
% Qwen2-500M & 13.4 & 14.0 & 14.1 & 14.1 & 791.2 & 784.5 & 816.1 & 912.0 \\
% \textbf{Ours (370M)} & \textbf{21.6} & \textbf{21.6} & \textbf{21.6} & \textbf{21.6} & \textbf{223.1} & \textbf{223.1} & \textbf{223.1} & \textbf{223.1} \\
\midrule
Prefill & 500 & 1000 & 2000 & 4000 & 500 & 1000 & 2000 & 4000 \\
\midrule
% Alireo-400M & 849.4 & 1620.4 & 2858.0 & 3152.8 & 11.7 & 7.8 & 5.8 & 6.8 \\
Alireo-400M & 849.4 & 1620 & 2858 & 3153 & 11.7 & 7.8 & 5.8 & 6.8 \\
% Pythia-410M & 610.5 & 2472.2 & 3985.5 & 5065.9 & 14.9 & 4.9 & 4.3 & 4.2 \\
% Qwen2-500M & 627.0 & 909.3 & 1513.7 & 2639.4 & 17.9 & 13.9 & 9.5 & 6.7 \\
Qwen2-500M & 627 & 909 & 1514 & 2639 & 17.9 & 13.9 & 9.5 & 6.7 \\
\textbf{Ours (370M)} & \textbf{13965} & \textbf{13965} & \textbf{13965} & \textbf{13965} & \textbf{2.8} & \textbf{2.8} & \textbf{2.8} & \textbf{2.8} \\
\bottomrule
\multicolumn{9}{p{12.5cm}}{
\tiny$^*$ The MatMul-free LM on Loihi 2 was characterized on an Oheo Gulch single-chip Loihi 2 system (N3C1 silicon) running NxKernel v0.2.0 and NxCore v2.5.8 (only accessible to Intel Neuromorphic Research Community members).
\par
$^\ddagger$ Transformer LMs characterized on NVIDIA Jetson Orin Nano 8GB using MAXN power mode running Jetpack 6.2, TensorRT 10.3.0, CUDA 12.4. Energy values include CPU\_GPU\_CV, SOC, and IO components as reported by jtop 4.3.0.
\par
Performance results as of Jan 2025 and may not reflect all publicly available security updates. Results may vary.
}
\end{tabular}
\label{tab:jetson-loihi-comp}
\end{table*}

Table~\ref{tab:jetson-loihi-comp} contrasts the estimated performance of the 370M MatMul-free model on Loihi 2 against transformer-based baselines running on an NVIDIA Jetson Orin Nano, showing at least 2x less energy per token for prefill, and at least 3x less energy per token for auto-regressive generation. Throughput for autoregressive generation is comparable across models, while for prefill the throughput of our MatMul-free LM on Loihi 2 is at least 4x higher. More details can be found in Appendix~\ref{app:l2-results-detailed}

\section*{Old results in Appendix C.4.1}

\begin{table*}[h]
\caption{Throughput and energy efficiency estimates for our MatMul-free LM running on Intel's Loihi 2, based on a 1-chip implementation and a 24-chip implementation. Each chip implements a single block of the language model. \textbf{GEN}: autoregressive generation, \textbf{PF}: prefill mode.}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{cl|cc}
\toprule
 && Throughput ($\uparrow$ tokens/sec) & Efficiency ($\downarrow$ mJ/token) \\
\midrule
\multirow{2}{*}{\rotatebox{90}{GEN}} &
% ./profiling/profiling_iclr-test-store-hicore-ap-24chip-tmp-ap01.html
\textbf{Ours (370M)} (24-chip) & \textbf{41.5} & \textbf{405} \\
& \textbf{Ours (370M)} (1-chip) & \textbf{71.3} & \textbf{59} \\
\midrule
\multirow{2}{*}{\rotatebox{90}{PF}} &
\textbf{Ours (370M)} (24-chip) & \textbf{6632} & \textbf{3.7} \\
& \textbf{Ours (370M)} (1-chip) & \textbf{13965} & \textbf{2.8} \\
\bottomrule
\multicolumn{4}{p{12.5cm}}{\tiny$^*$ MatMul-free LM on Loihi 2 on (1) Oheo Gulch single-chip Loihi 2, (2) Alia Point 32-chip Loihi 2 (both: N3C1 silicon) running NxKernel v0.2.0 and NxCore v2.5.8 (accessible to Intel Neuromorphic Research Community members).
\par
$^\dagger$ Transformer LMs were characterized on NVIDIA Jetson Orin Nano 8GB, MAXN power mode, Jetpack 6.2, TensorRT 10.3.0, CUDA 12.4. Energy values include CPU\_GPU\_CV, SOC, and IO components as reported by jtop 4.3.0.
\par
Performance results as of Jan 2025 and may not reflect all publicly available security updates. Results may vary.
}
\end{tabular}
}
\label{tab:loihi-table-1-24-chip}
\end{table*}

\paragraph{Limitations and further optimizations}
Ongoing optimization efforts target latency and power reduction for the MatMul-free LM on Loihi 2. We anticipate 24-chip system energy efficiency approaching single-chip estimates (Table \ref{tab:loihi-table-1-24-chip}).
